Dark Memory and Accelerator-Rich System Optimization in the Dark Silicon Era

The key challenge to improving performance in the age of Dark Silicon is how to leverage transistors when they cannot all be used at the same time. In modern SOCs, these transistors are often used to create specialized accelerators which improve energy efficiency for some applications by 10-1000X. While this might seem like the magic bullet we need, for most CPU applications more energy is dissipated in the memory system than in the processor: these large gains in efficiency are only possible if the DRAM and memory hierarchy are mostly idle. We refer to this desirable state as Dark Memory, and it only occurs for applications with an extreme form of locality. To show our findings, we introduce Pareto curves in the energy/op and mm$^2$/(ops/s) metric space for compute units, accelerators, and on-chip memory/interconnect. These Pareto curves allow us to solve the power, performance, area constrained optimization problem to determine which accelerators should be used, and how to set their design parameters to optimize the system. This analysis shows that memory accesses create a floor to the achievable energy-per-op. Thus high performance requires Dark Memory, which in turn requires co-design of the algorithm for parallelism and locality, with the hardware.

==> Notes.tex <==
\begin{color}{red}

\vspace{2\baselineskip}

TODO
\begin{itemize}
    \item paste mh outline below
    \item make a skeleton for the new paper
\end{itemize}

\vspace{2\baselineskip}

NOTES
\begin{itemize}
    \item people authorized to do aggressive edits and decision making: ardavan and mark (right, mark/ardavan?)
  
    \item collaborators: shahar, steve, sameh, others \\
    (right, mark/ardavan?)
  
\end{itemize}

\vspace{2\baselineskip}

% \begin{verbatim}
% other notes
% \end{verbatim}

\end{color}


==> Outline.tex <==
\begin{footnotesize}
\setlength{\parindent}{0cm}
% \setlength{\parskip}{\baselineskip}

\vspace{\baselineskip}
1. Introduction – 1 page

i. Quick review of scaling issues that got us into this issue
\vspace{\baselineskip}

% \hangindent=0.5cm
\setlength{\parindent}{0.5cm}
\parindent 0.2cm
  1. While Dennard scaling showed how to scale CMOS devices at constant power density, CMOS processor chip power grew exponentially from the mid 80 to the late 90s since we were scaling clock frequency faster than 1/L, and voltages slower than L.  By the mid 2000’s all computing systems, even high-end servers, ran into power limitations, which meant that further performance increases could not increase the power of the system.

  2. During this same period, voltage scaling essentially stopped.  Now scaling to a new technology only scales the gate energy by L (not $L^3$), so if you build $L^{-2}$ processors (to use all transistors available in the same area), and run them at the same frequency, the power will go up by $L^{-1}$ which is not allowed

  3. This  means that you can’t run all the transistors on your chip at the same time as you previously had done, which gave rise to the term Dark Silicon – transistors on the die that can’t be used (at this time) for power reasons. 

  4. This paper will review some of the issues and approaches for creating high-performance computing platforms in the Dark Silicon Era

%\end{quote}
\vspace{\baselineskip}
\begin{quote}

ii. Clearly building transistors that are never used is silly.  Michael Taylor, in his Four Horsemen of Dark Silicon paper [ref] proposed four better solutions: shrink, dim, specialize, magic

\begin{quote}

  1. If you can’t use the transistors, don’t build them and just shrink the die.  It’s power density will go up, but the package/heatsink won’t change much (since it goes in the same user device, and will be able to handle the heat.  Power density of the chip is not really the issue.  This makes the computing device cheaper to manufacture, but its performance won’t improve much.

  2. Another option, dim, is to try to lower the power/gate by lowering the frequency.
  
  \begin{quote}

    2-1.  At first this seems to make sense, since now we can use all the transistors, but simple frequency scaling is silly.  To get the same performance we need more cores, and  if the energy/instruction hasn’t changed, the overall performance won’t change: Power = energy/s = energy/instr * instr/sec.  So we get the same performance as before, but now we use more silicon area.  That’s dumb. 

    2-2. For dim to work, we need to decrease the energy/inst as we slow it down, which people usually assume will be done by voltage scaling, or simpler architectures.  This does work, and these techniques have been used in the transition to multi-core designs to allow us to scale to 4-8 processors. Modern processors have very aggressive voltage/frequency scaling.  These systems are running at so low margins already that they need to lower their clock frequency when they detect a small glitch in their supply voltage. 

    2-3. Unfortunately as we will see in Section XXX there is a law of diminishing returns, so further lowering the energy/op by voltage/microarchitecture is very hard today.

  \end{quote}
  \vspace{\baselineskip}
  \begin{quote}


3. Magic, or the Dues Ex Machina Horseman, requires a dramatic change in the underlying device technology

3-1. While it would be great if a new better technology/approach is found, we shouldn’t count on it for two reasons. First it is unlikely:

3-2. While I am sure we can easily accommodate any type of device that looks like a transistor, devices that look like transistors have the same physical limitation as todays devices, and will have the same voltage limitation. To get around these limitations the device will have to be very different, and the economic cost of creating both the manufacturing facility and the design community to deal with this very different device seems very large.  Getting very large money for very different and thus risky ideas is hard.

3-3. Second, it abdicates our role in helping to continue to improve computing.

  \end{quote}
  \vspace{\baselineskip}
  \begin{quote}


4. That leaves specialization as the principle viable method to improve computing performance

4-1. There are many examples of specialized hardware being many orders of magnitude more efficient than CPUs, so many people think this is the magic bullet.

4-2. Yet when you look at the energy dissipation in a CPU chip, around ½ of it is in the memory system, and from a system perspective the ratio is even worse, since the system power must include the DRAM energy as well.

4-3. If this is the case didn’t Amdahl said something about the maximum potential energy saving by changing the compute unit a long time ago? 

4-4. The truth is specialization only works when the application has very good locality, so that most of the memory hierarchy is idle almost all of the time. We will call this Dark Memory, and it is to first order a function of the locality of the algorithm used, and then how well the hardware captures this locality.

  \end{quote}
  \vspace{\baselineskip}
  \begin{quote}



iii. This papers explores techniques for designing in the Dark Silicon Era.  

1. To enable us to optimize these dark silicon systems with multiple specialized cores, we need metrics to evaluate the resulting systems.  Section 2 describes how to use energy/op, and op/(s*mm$^2$) to fairly compare two power constrained systems, and explains why these are the best metrics to use.

2. Using these metrics, Section 3 then explores the ramifications of the high energy cost of memory fetches, and how this energy changes with the size of the working set. The unavoidable conclusion is that most of the system memory must be dark to achieve good energy efficiency.

3. Given this insight, Section 4 describes the critical design loop for Dark Silicon systems, the co-optimization between the algorithm, compute and memory system design. We need to first find an algorithm with good locality, and then find hardware compute and memory structures that exploit it.

4. To tie these three design tasks together, Section 5 formulates the design optimization problem for the Dark Silicon Era: given a set of proposed workloads, draw the Pareto curve of average system energy, and average system area efficiency while guaranteeing that all critical traces meet their performance and power constraints.

\end{quote}

2. Metrics for energy constrained computing (1.5 pages)

i. In the design of any piece of hardware (or software) there are many different choices the designer can make.  Each will yields a different design.  While some design choices are binary (example), others take a range of values (depth of pipelining, width of SIMD unit, \# of registers). These design choices parameterize the design space. Recently the notion of hardware constructors, or generators implemented this abstraction of a parameterized design space (could be a footnote).  When we were focused on performance, the objective was clear, and hence the metric was clear: system performance.  

ii. In the Dark Silicon Era, performance is still important, but so is energy/op.  This raises the question of the best metric space to use to compare two different designs.  This metric space should allow us to compare performance, power, and die cost of our design.  (Silicon might be cheap, but it is not free when you sell 10$^7$ chips).  Power affects the system in two ways: can’t dissipate too much power for two long, because you get to hot, and extended battery life.  The first one is usually more critical. Generally limited by getting the heat out of the system, not the chip – heat pipes are pretty good.

iii. In chip design there is a tendency to focus on the chip, or subsystem being designed.  But the metrics need to include the entire system being used, especially, as we will see in Section 3, the memory system

b. Energy and area metric space

i. Clearly getting low energy/op is critical, since power= performance *energy/op.  But we also need a solution that generates high performance.  Minimizing energy/op yields very slow systems.  Need to add a performance constraint. Most efficient solutions are parallel, so the performance of a single unit is not that critical, could use multiple units instead.  What you care about is the silicon cost to achieve that performance, or mm^2/(ops/s), to make sure we can get the performance we need in the available silicon area.  Note that the granularity of an op (instruction, arithmetic operation, processing a whole image) doesn’t change the optimization problem, and can be chosen to make computing the numbers as simple as possible.1 

ii. Create the Pareto curve in the energy/op, and mm^2/(ops/s). (Figure 2a) All designs that are not on this curve are strictly worse that another design on the curve.  Show why. Which point on the curve is best depends on your objectives

iii. Draw Figure 2b, and explain how the different types of constraints easily fix on this graph.  Then show that the lines of constant performance are just scaled versions of the Pareto curve in 2a.

c. Finding Optimal Designs

i. Explain how to compute the max throughput for an area/power constrained design

ii. Then show how any optimization problem simply becomes a line in this metric space, and you are trying to find the max line that intersects with the Pareto curve

iii. The previous idea will take a couple of paragraphs

iv. Previous idea

d. Multiple unit optimization 2

i. Previous method was looking at one design, but the same idea works for an application that requires multiple accelerators.  Now the chip area has to be the sum of the areas of the accelerators (but be careful not to double count shared memory structures)

ii. The performance is the performance of the whole application, and not the performance of the part of the application running on the accelerator.  Simple formula to generate this curve from component curves.3 

iii. This formulation makes it possible to compare to separate accelerators vs an accelerator that is more general, but less efficient than it completely specialize accelerators

iv. An example showing the previous example, perhaps a GEMM and FFT accelerators, and then a combined accelerator.  This might take 3 paragraphs

3. Why Dark Memory is Essential (< 1.5 pages)

i. It is well known in a modern CMOS technology computation is pretty energy efficient, it is communication that requires larger amount of energy.  Memory lookup is a form of communication (explain). Length of communication is related to the size of the memory.

b. Memory energy

i. Memory energy are large compared to simply ops - Have operation energy table

ii. Energy cost of a simple instruction, maximum potential energy advantage if the code does a number of L1 level fetches

iii. Energy/bit depends on the fetch width.  Wider fetches are better - explain

iv. SRAM are never completely dark.  Talk about SRAM leakage, what it depends on, and current values

v. Potential new memory technology and how that may change the numbers

vi. Potential memory continued

c. Power limited memory intensive applications

i. The same optimization formulations works for this applications as well.  Still measure energy/op, and mm^2/(op/s).  Only difference might be in the choice of “op”

ii. Changing all the different memory sizes yields a Pareto curve for your system. Explain how that works

iii. Memories are large, often consuming large % of area.  Thus they are generally shared between different cores when possible.  This also helps with the leakage energy

iv. But the energy cost of memory forms strong limits on the performance of the memory intensive applications.  Parallel memories don’t reduce energy/fetch, there is a limit of fetches.  Give the max number of L1 L2 L3 and DRAM fetches/W.  

v. Another way of looking at this is what miss rate is required so high-level memory doesn’t dominate memory energy.

4. The Co-design Triangle (.75 pages)

i. Previous section showed the importance of memory behavior to energy/op.  Yet the cache hit rates are really set by the locality structure of the application.  Introduce working set and reuse distance.

ii. Efficient hardware also requires data parallelism to achieve the high ops rates that modern applications demand.

iii. Generating this locality and parallelism requires changes to the algorithm used for the application.  In fact much of the work done when creating an ASIC implementation of a function is really these application changes.  It would be great to have some examples.  I think there are some in Wajahat and Rehan’s first paper

iv. For certain classes of applications, there are languages that are being developed to help with some of this optimization.  Talk about Halide for image processing which separates out the schedule, and how this changes computation and memory locality

v. And some of the linear algebra systems (auto tuners?) 

vi. For each of the algorithm variant created, we can first construct a Pareto curve for the hardware/memory system design as was described in Section 2. This curve would represent the hardware and memory system parameters that are on the optimal boundary for energy (energy/op) and compute density (mm^2/(op/s)).  To create the actual Pareto curve, the curve for each algorithmic variant is computed, and the boundary curve of all these curves becomes the Pareto curve for the joint algorithm/hardware/memory optimization.

5. Dark silicon system optimization (.75 page)

i. Given our metric space and our ability to find the Pareto optimal curve for all algorithmic and hardware parametric choices, it might at first seem like the overall hardware/software optimization problem would be simple to state/solve: create the weighted average Pareto optimal curve for your application mix, and then choose the point on the curve which optimizes your “cost” function.  This is the method describes in Section 2.3.  While this is roughly correct, there are a number constraints and complexity that needs to be considered.

b. Scenario Constraints

i. Not only do we want to optimize the weighted average of all application scenarios, we need to ensure that each scenario can achieve a min performance within the power budget.  What does this mean?  We need to figure it out.  I think it means we generate the Pareto curves for each of the specialized accelerators. Next we need to create the Pareto curve for the average cost.  But now we are constrained never to choose parameters for any of the units that would cause another trace to exceed its boundary, so it might remove some of the points from the unconstrained optimization.

ii. Further discussion of this problem

iii. Probably one more

iv.  It would be great if we could work out a problem

c. Shared hardware

i. While the individual scenario constraints made the merging of the Pareto curves more complex, it still could leverage the curves generated for each accelerator to create its final result.  When multiple specialized hardware units share some of the hardware blocks, generally the higher levels in the memory hierarchy, the underlying trade-off curves change.  Some of the area is being used in two modules, so only a fraction of it should be charged for each module.  Explain this only happens if the units are not simultaneously running, since then the size of the memory would need to grow and the area savings is smaller.

ii. While solving this in general can be hard, it is easy to pull the memory system out, and generate Pareto curve for each accelerator as a function of the memory system.  Using this we can use this to create the optimal designs.

iii. This needs more work, but my brain needs a break.

6. Conclusion


1 But you want the op to be related to the application objectives.  You would like a better algorithm which takes fewer multiplies to have a lower energy/op, which might not be the case if your op was multiplies.

2 But this is for a single application, which makes it much simpler

3 Need to double check the Pareto curve designs are still optimal, but I am pretty sure they are
---------------

------------------------------------------------------------

---------------

------------------------------------------------------------
\end{small}


==> Pareto.tex <==
\begin{normalsize}
\setlength{\parindent}{0cm}

% 
\color{green}
% 
5. Dark silicon system optimization (.75 page)

\vspace{\baselineskip}
a-i. Given our metric space and our ability to find the Pareto optimal curve for all algorithmic and hardware parametric choices, it might at first seem like the overall hardware/software optimization problem would be simple to state/solve: create the weighted average Pareto optimal curve for your application mix, and then choose the point on the curve which optimizes your “cost” function.  This is the method describes in Section 2.3.  While this is roughly correct, there are a number constraints and complexity that needs to be considered.

\vspace{\baselineskip}
b. Scenario Constraints

b-i. Not only do we want to optimize the weighted average of all application scenarios, we need to ensure that each scenario can achieve a min performance within the power budget.  What does this mean?  We need to figure it out.  I think it means we generate the Pareto curves for each of the specialized accelerators. Next we need to create the Pareto curve for the average cost.  But now we are constrained never to choose parameters for any of the units that would cause another trace to exceed its boundary, so it might remove some of the points from the unconstrained optimization.

b-ii. Further discussion of this problem

b-iii. Probably one more

b-iv.  It would be great if we could work out a problem

\vspace{\baselineskip}
c. Shared hardware

c-i. While the individual scenario constraints made the merging of the Pareto curves more complex, it still could leverage the curves generated for each accelerator to create its final result.  When multiple specialized hardware units share some of the hardware blocks, generally the higher levels in the memory hierarchy, the underlying trade-off curves change.  Some of the area is being used in two modules, so only a fraction of it should be charged for each module.  Explain this only happens if the units are not simultaneously running, since then the size of the memory would need to grow and the area savings is smaller.

c-ii. While solving this in general can be hard, it is easy to pull the memory system out, and generate Pareto curve for each accelerator as a function of the memory system.  Using this we can use this to create the optimal designs.

c-iii. This needs more work, but my brain needs a break.

\begin{footnotesize}

